Towards 3D Scene Understanding by Referring Synthetic Models

Promising performance has been achieved for visual perception on the point cloud. However, the current methods typically rely on labour-extensive annotations on the scene scans. In this paper, we explore how synthetic models alleviate the real scene annotation burden, i.e., taking the labelled 3D synthetic models as reference for supervision, the neural network aims to recognize specific categories of objects on a real scene scan (without scene annotation for supervision). The problem studies how to transfer knowledge from synthetic 3D models to real 3D scenes and is named Referring Transfer Learning (RTL). The main challenge is solving the model-to-scene (from a single model to the scene) and synthetic-to-real (from synthetic model to real scene's object) gap between the synthetic model and the real scene. To this end, we propose a simple yet effective framework to perform two alignment operations. First, physical data alignment aims to make the synthetic models cover the diversity of the scene's objects with data processing techniques. Then a novel \textbf{convex-hull regularized feature alignment} introduces learnable prototypes to project the point features of both synthetic models and real scenes to a unified feature space, which alleviates the domain gap. These operations ease the model-to-scene and synthetic-to-real difficulty for a network to recognize the target objects on a real unseen scene. Experiments show that our method achieves the average mAP of 46.08\% and 55.49\% on the ScanNet and S3DIS datasets by learning the synthetic models from the ModelNet dataset. Code will be publicly available.

==> future.tex <==
\section{Future Work}


\begin{itemize}
\item {\textbf{training with multiple GPUs}}
\item {\textbf{add full classes.}}
\item {\textbf{add more datasets.}}
\item {add virtual scanning}
\item {\textbf{zero-shot setting. During infering time. given unseen referring models, localize the same semantic objects in an unseen scene}}
\item {visualization of prototypes}
\item {more downstream tasks}
\item {visualization of data processing}
\item {T-SNE visualization}
\item {Teacher student network, teacher for virtual data, student for real data}
\item {herchial memory for inner class and inter class}
\item {adjust temperature to synthe new features}
\item {reuse the classifier to fine-tune}
\item {voxel transformer}
\item {contrastive learning between models}

\end{itemize}

==> sup.tex <==

PointContrast (\cite{xie2020pointcontrast}) extends contrastive learning technique for learning point-wise representations that are beneficial to various downstream tasks. ADDA \cite{tzeng2017adversarial} utilize the generative adversarial networks to perform domain adaptation. PointDAN \cite{qin2019pointdan} jointly aligns the global and local features via adversarial-training strategy and self-adaptive node. However, the above methods are not suitable for this problem. 




\begin{table}[h]
    %\scriptsize
	\centering
	%\vspace{-1ex}
	\caption{Fine-tuning on the Scannet and S3DIS dataset. We omit the \% to show the IoU performance. The number in () donates the improved accuracy compared with purely supervised training.}\label{tab:fineTuning}
	\scalebox{0.75}{
	\begin{tabular}{l|l|c c c}
		\hline
        \multirow{2}*{\tabincell{c}{Dataset}} &
		\multirow{2}*{\tabincell{c}{Model}} &
		\multirow{2}*{\tabincell{c}{5\%  data}} &
		\multirow{2}*{\tabincell{c}{10\% data}} &
		\multirow{2}*{\tabincell{c}{100\%  data}}\\
		%\multirow{2}*{\tabincell{c}{VGG19\_bn}} &  \multicolumn{10}{c|}{~}\\
		~&~ & ~&~& ~ \\

        \hline
		\multirow{3}*{\tabincell{c}{Scannet}}&Trained from scratch  & 50.24 & 54.86 & 63.05 \\
		~&PointContrast \cite{xie2020pointcontrast}  & 55.31(5.07) & 58.68(3.82) & \textbf{65.03(1.98)} \\
		~&Ours & \textbf{56.12(5.88)} & \textbf{59.03(4.17)} & 64.93(1.88) \\

		\hline
		\multirow{3}*{\tabincell{c}{S3DIS}}&Trained from scratch &~& ~& ~56.44\\
		~&PointContrast \cite{xie2020pointcontrast} &~& ~& ~58.65(2.21) \\
		~&Ours &~& ~& ~\textbf{58.89(2.63)} \\
	\end{tabular}}
	%\vspace{-1ex}
\end{table}


\begin{table}[h]
    %\scriptsize
    \setlength{\tabcolsep}{0.2mm}
	\centering
	\caption{Fine-tuning on the Scannet dataset. We omit the \% to show the performance. The number in () donates the improved accuracy compared with purely supervised training.}\label{tab:fineTuning_scannet}
	\scalebox{0.8}{
	\begin{tabular}{c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{5\% data} &
		\multirow{2}*{10\% data} &
		\multirow{2}*{50\% data} &
		\multirow{2}*{100\% data} &

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Trained from scratch & 50.24 & 54.86 & 59.76 & 63.05 \\
	    PointContrast \cite{xie2020pointcontrast} & - & -& - & - \\
	    Ours & 56.12(5.88) & 59.03(4.17)& 62.00(2.24) & 64.93(1.88) \\

	\end{tabular}}
\end{table}

\begin{table}[h]
    %\scriptsize
    \setlength{\tabcolsep}{0.8mm}
	\centering
	\caption{Fine-tuning on the S3DIS dataset. We omit the \% to show the performance. The number in () donates the improved accuracy compared with purely supervised training.}\label{tab:fineTuning_S3DIS}
	\scalebox{0.8}{
	\begin{tabular}{c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{5\% data} &
		\multirow{2}*{10\% data} &
		\multirow{2}*{50\% data} &
		\multirow{2}*{100\% data} &

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Trained from scratch & - & - & - & - \\
	    PointContrast \cite{xie2020pointcontrast} & - & -& - & - \\
	    Ours & - & -& - & - \\

	\end{tabular}}
\end{table}


\begin{table*}[h]
    %\scriptsize
	\centering
	%\vspace{-1ex}
	\caption{Zero-shot experiments on scannet dataset.}\label{tab:zero_shot}
	\scalebox{0.93}{
	\begin{tabular}{l|c c c c c c c l|c c c c c}
        \hline
		\multirow{2}*{\tabincell{c}{Model}} &
        \multicolumn{8}{c}{Seen classes} & \multicolumn{5}{c}{Unseen classes}\\
        \cline{2-14}

		~ & chair & table & bed & sink & bathtub & door & curtain & AmAP & desk & bookshelf & sofa & toilet & AmAP\\
        \hline
		FSL & 91.44 & 72.89 & 76.35 & 83.94 & 84.84  & 58.47 & 74.22 & 77.45 & 72.96 & 75.76 & 84.81 & 93.10  & 81.65\\
		DeViSe \cite{frome2013devise} & 88.01 & 69.10 & 75.10 & 80.38 & 79.74 & 52.59 & 66.09 & 73.01 & 24.28 & 11.92 & 20.36 & 1.96  & 14.63\\
		GZSL \cite{michele2021generative} \\
		
		Ours & 87.53 & 66.70 & 73.53 & 78.37 & 83.05 & 46.94 & 62.94 & 71.29 & 21.53 & 12.33 & 34.42 & 7.76  & 19.01\\

	\end{tabular}}
	%\vspace{-1ex}
\end{table*}



\begin{table}[h]
    %\scriptsize
	\centering
	\caption{Evaluation on the S3DIS. MinkUNnet is the baseline method. GT indicates training with ground truth. }\label{tab:S3DIS}
	\scalebox{0.83}{
	\begin{tabular}{c c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{AmAP} &
		\multirow{2}*{chair} &
		\multirow{2}*{bookshelf} &
		\multirow{2}*{sofa} &
		\multirow{2}*{table} &

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Baseline & 15.65 & 3.75 & 37.72 & 13.34 & 7.80\\
        ADDA \cite{tzeng2017adversarial} & 26.57  & 26.67& 54.70 & 15.91 & 9.00 \\
        ADDA$\dagger$ \cite{tzeng2017adversarial} & 30.04  & 57.80 & 54.70 & 22.91 & 8.70 \\
	    PointDAN \cite{qin2019pointdan} & 39.80 & 56.60& 52.34 & 32.06 & 18.20 \\
	    3DIoUMatch \cite{wang20213dioumatch} & 49.60 & 69.07 & 56.87 & \textbf{54.25} & 18.21 \\
	    Ours & \textbf{55.49} & \textbf{70.86} & \textbf{62.68} & 47.87 & \textbf{40.57} \\
        \hline
	    GT & 90.44 & 97.05 & 87.84 & 86.83  & 90.06  \\
	    GT+ours & 92.57 & 97.83 & 89.86 & 92.05 &  90.52 \\

	\end{tabular}}
\end{table}



\begin{table*}[h]
    %\scriptsize
	\centering
	\caption{Evaluation on the ScanNet. MinkUNnet is the baseline method. GT indicates training with ground truth. }\label{tab:Scannet}
	\scalebox{0.91}{
	\begin{tabular}{c c c c c c c c c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{AmAP} &
		\multirow{2}*{chair} &
		\multirow{2}*{table} &
		\multirow{2}*{bed} &
		\multirow{2}*{sink} &
		\multirow{2}*{bathtub} &
		\multirow{2}*{door} &
		\multirow{2}*{curtain} &
		\multirow{2}*{desk} &
		\multirow{2}*{bookshelf} &
		\multirow{2}*{sofa} &
		\multirow{2}*{toilet} &


		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Baseline & 10.93 & 8.09 & 10.60 & 15.97 & 2.53 & 12.40 & 9.77 & 13.92 & 4.66 & 26.76 & 11.49 & 4.07\\
        ADDA \cite{tzeng2017adversarial} & 28.93 & 29.93 & 40.88 & 36.82 & 8.03 & 31.60 & 13.59 & 25.10 & 20.01 & 35.49 & 33.90 & 42.92 \\
        ADDA$\dagger$ \cite{tzeng2017adversarial} & 38.14 & 67.03 & \textbf{48.60} & 29.77 & 20.36 & 29.70 & 12.04 & 23.06 & 26.57 & 42.69 & 51.41 & 68.31 \\
	    PointDAN \cite{qin2019pointdan} & 32.92 & 58.31 & 40.39 & 20.96 & 12.58 & 31.65  & 11.79 & 17.65 & 26.04 & 48.31 & 41.25 & 53.18 \\
	    3DIoUMatch \cite{wang20213dioumatch} & 42.25 & 63.34 & 41.24 & 43.58 & 26.53 & \textbf{46.61} & 15.52 & 24.45 & 26.75  & 45.49 & 54.49 & \textbf{76.81} \\
	    Ours & \textbf{46.08} & \textbf{67.19}& 46.73 & \textbf{45.65}& \textbf{31.28} & 43.36 & \textbf{17.47} & \textbf{34.43} & \textbf{29.15} & \textbf{59.37} & \textbf{60.48} & 71.77\\
        \hline
	    GT & 78.98  & 91.44 & 72.89 & 76.35 & 83.94 & 84.84  & 58.47 & 74.22 & 72.96 & 75.76 & 84.81 & 93.10 \\
	    Ours+GT & 79.46  & 92.16  & 74.37  & 76.50  & 85.18 & 85.09 & 56.57 & 70.68 & 73.54 & 77.03 & 87.44 & 95.52\\

	\end{tabular}}
\end{table*}



\begin{table*}[h]
    %\scriptsize
	\centering
	\caption{Ablation experiments. MinkUNnet is the baseline method. Mix and FA donate point mixing up and feature alignment by the prototypes, respectively.}\label{tab:ablation}
	\scalebox{0.84}{
	\begin{tabular}{c c c c c c c c c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{AmAP} &
		\multirow{2}*{chair} &
		\multirow{2}*{table} &
		\multirow{2}*{bed} &
		\multirow{2}*{sink} &
		\multirow{2}*{bathtub} &
		\multirow{2}*{door} &
		\multirow{2}*{curtain} &
		\multirow{2}*{desk} &
		\multirow{2}*{bookshelf} &
		\multirow{2}*{sofa} &
		\multirow{2}*{toilet} &


		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    MinkUNet & 10.93 & 8.09 & 10.60 & 15.97 & 2.53 & 12.40 & 9.77 & 13.92 & 4.66 & 26.76 & 11.49 & 4.07\\
	    \hline
	    MinkUNet+Mix$_{noDA}$ & 23.44 & 36.90 & 35.57 & 26.30 & 11.98 & 17.29 & 11.01 & 21.07 & 11.58 & 25.03 & 16.40 & 44.66 \\
	    MinkUNet+Mix$_{negaSc}$ & 23.04  & 41.74 & 25.05 & 21.92 & 7.86  & 23.01 & 13.88 & 21.93 & 14.79 & 23.80 & 13.08 & 46.39 \\
	    MinkUNet+Mix$_{negaMo}$ & 41.34 & \textbf{73.12} & 40.05 & 42.73 & 29.17  & 19.97 & 17.52 & 23.33 & 33.40 & 50.34 & 59.36 & 65.71 \\
	    MinkUNet+Mix$_{negaMo\_noCo}$ & 37.83 & 72.62 & 39.61 & 37.49  & 14.95 & 16.93 & 18.33 & 21.29 & 32.84 & 46.09 & 59.44 & 56.53 \\
	    
	    MinkUNet+Mix & 42.19 & 67.53 & 47.64 & 41.82  & 27.01  & 32.47  & 13.68  & 27.82  & 26.78  & 50.54  & 58.75  & 70.07 \\
        \hline
        MinkUNet+Mix+FA$_{K64}$ & 43.16 & 67.37  & \textbf{48.27}  & 41.51  & 20.38 & 33.90 & 16.30  & 31.55  & 27.17  & 52.32  & \textbf{61.19}  & 74.84  \\
	    MinkUNet+Mix+FA$_{K128}$ & \textbf{46.08} & 67.19& 46.73 & 45.65& \textbf{31.28} & 43.36 & 17.47 & 34.43 & 29.15 & \textbf{59.37} & 60.48 & 71.77\\
        MinkUNet+Mix+FA$_{K256}$ & 43.81 & 68.15  & 45.12 & \textbf{51.08} & 20.12 & 38.14 & 17.10 & 25.64 & \textbf{33.99} & 48.23 & 59.32  & 75.05 \\
	    MinkUNet+Mix+FA$_{T4}$ & 44.51 & 69.05 & 47.28 & 49.72 & 18.26  & \textbf{45.30} & \textbf{18.46} & 28.83 & 26.16 & 49.94 & 57.23 & \textbf{79.40} \\
	    MinkUNet+Mix+FA$_{T0.1}$ & 43.79 & 70.47 & 42.44 & 44.26 & 20.95 & 39.57 & 16.00 & 29.92 & 27.65 & 52.04 & 59.14  & 79.20\\
	    MinkUNet+Mix+FA$_{cos}$  & 43.45  & 69.16  & 45.84 & 42.53  & 21.47 & 37.38 & 15.36 & 29.20 & 29.06 & 51.72 & 59.16 & 77.06\\
	    MinkUNet+Mix+FA w/o WE  & 44.84 & 70.06 & 46.98 & 45.27 & 23.25  & 36.52 & 17.29 & \textbf{45.11} & 33.97 & 50.90  & 56.43 & 67.41\\


	\end{tabular}}
\end{table*}

\begin{table}[h]
    %\scriptsize
    \setlength{\tabcolsep}{0.2mm}
	\centering
	\caption{Fine-tuning on the Scannet dataset. We omit the \% to show the performance. The number in () donates the improved accuracy compared with purely supervised training.}\label{tab:fineTuning_scannet}
	\scalebox{0.8}{
	\begin{tabular}{c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{5\% data} &
		\multirow{2}*{10\% data} &
		\multirow{2}*{50\% data} &
		\multirow{2}*{100\% data} &

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Trained from scratch & 50.24 & 54.86 & 59.76 & 63.05 \\
	    PointContrast \cite{xie2020pointcontrast} & - & -& - & - \\
	    Ours & 56.12(5.88) & 59.03(4.17)& 62.00(2.24) & 64.93(1.88) \\

	\end{tabular}}
\end{table}

\begin{table}[h]
    %\scriptsize
    \setlength{\tabcolsep}{0.8mm}
	\centering
	\caption{Fine-tuning on the S3DIS dataset. We omit the \% to show the performance. The number in () donates the improved accuracy compared with purely supervised training.}\label{tab:fineTuning_S3DIS}
	\scalebox{0.8}{
	\begin{tabular}{c c c c c}
        \hline
%         \multirow{2}*{backbone} &
% 		\multirow{2}*{attention strategy} &
        \multirow{2}*{Method} &
		\multirow{2}*{5\% data} &
		\multirow{2}*{10\% data} &
		\multirow{2}*{50\% data} &
		\multirow{2}*{100\% data} &

		~ & ~ \\
% 		\hline
% 	    baseline & - \\
	    \hline
	    Trained from scratch & - & - & - & - \\
	    PointContrast \cite{xie2020pointcontrast} & - & -& - & - \\
	    Ours & - & -& - & - \\

	\end{tabular}}
\end{table}

